SLING: Sino Linguistic Evaluation of Large Language Models

To understand what kinds of linguistic knowledge are encoded by pretrained Chinese language models (LMs), we introduce the benchmark of Sino LINGuistics (SLING), which consists of 38K minimal sentence pairs in Mandarin Chinese grouped into 9 high-level linguistic phenomena. Each pair demonstrates the acceptability contrast of a specific syntactic or semantic phenomenon (e.g., The keys are lost vs. The keys is lost), and an LM should assign lower perplexity to the acceptable sentence. In contrast to the CLiMP dataset (Xiang et al., 2021), which also contains Chinese minimal pairs and was created by translating the vocabulary of the English BLiMP dataset, the minimal pairs in SLING are derived primarily by applying syntactic and lexical transformations to naturally-occurring, linguist-annotated sentences from the Chinese Treebank 9.0, thus addressing severe issues in CLiMP's data generation process. We test 18 publicly available pretrained monolingual (e.g., BERT-base-zh, CPM) and multi-lingual (e.g., mT5, XLM) language models on SLING. Our experiments show that the average accuracy for LMs is far below human performance (69.7% vs. 97.1%), while BERT-base-zh achieves the highest accuracy (84.8%) of all tested LMs, even much larger ones. Additionally, we find that most LMs have a strong gender and number (singular/plural) bias, and they perform better on local phenomena than hierarchical ones.

==> sections/phenomena.tex <==
\section{Phenomena}\label{sec.phenomena}

\dataset~includes 9 major Chinese linguistic phenomena in syntax and semantics, summarized in Table \ref{tab:overview_phenomena}. Several minimal pair paradigms are designed to test the LMs' robustness to distance and distractor in a dependency relation as well as whether they have the hierarchy knowledge of Chinese. The details are offered in Appendix \ref{appendix.linguistic.phenomena}. Here we describe the gist of each phenomenon. The \textbf{alternative question} phenomenon tests the knowledge that the disjunctor \textit{haishi} and the polar question marker \textit{ma} may not co-occur. In the \textbf{anaphor agreement} phenomenon, we first use baselines to test the LMs' gender and number bias. Then, the morpheme \textit{ziji} (self) is added to test if the LMs knows the function of \textit{ziji} and agree the gender/number of the reflexive to the sentence subject. The \textbf{aspect} phenomenon tests the knowledge of the perfective aspect markers \textit{le} and \textit{guo} in the sense of their interaction with tense and the progressive marker \textit{zai}. The \textbf{classifier-noun agreement} occurs when a noun is modified by a numeral or demonstrative. One noun can be compatible with more than one classifier and the matching is idiosyncratic. The \textbf{definiteness effect} phenomenon is established on the observation that demonstrative \textit{zhe} (this)/\textit{na} (that) and the quantifier \textit{mei} (every) may not occur in the postverbal position of an existential \textit{there}-sentence. The \textbf{polarity item}s (PI) are the words/phrases whose occurrence is restricted to certain contexts (e.g., negative or affirmative). We test two negative PIs, \textit{renhe} (any) and \textit{shenme} (what), as well as one positive PI \textit{huoduo huoshao} (more or less). Chinese \textbf{relative clauses} exhibit a filler-gap dependency relationship. If the gap is a simple subject or direct object position, no resumptive noun or pronoun is allowed. Lastly, there is the \textbf{\textit{wh}-fronting} phenomenon, which shows that without being in a specific context (e.g., an echo question), a \textit{wh} phrase must stay in situ. 

\begin{table*}[!t]
\fontsize{8}{10}\selectfont
\centering 
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}p{1.5cm}p{7cm}p{7.5cm}ccccc@{}}
\toprule
\textbf{Phenomenon}    &  
\textbf{Acceptable Example}  & 
\textbf{Unacceptable Example} & 
\textbf{Syn} & 
\textbf{Sem} & 
\textbf{Distractor} & 
\textbf{Distance} & 
\textbf{Hierarchy}  \\
\midrule
Alternative Question & 
tamen shi laoshi ~~haishi mujiang? \newline they ~~~are teacher or ~~~~~~carpenter \newline ``Are they teachers or carpenters?'' &
tamen shi laoshi ~~haishi mujiang ~~\textbf{ma}? \newline they ~~~are teacher or ~~~~~~carpenter \texttt{SP} &
\ding{51} &           &            &     &     \\

\rowcolor{aliceblue}
 Anaphor \newline (Gender) & 
    nan ~~dianyuan ~~~~~~~kanjianle ~~\textbf{ta}-ziji.\newline male shop assistant saw ~~~~~~~~~~himself\newline
    ``The male shop assistant saw himself."& 
 nan ~~dianyuan ~~~~~~~kanjianle ~~\textbf{ta}-ziji.\newline male shop assistant saw ~~~~~~~~~~herself &
 \ding{51} &           & \ding{51} &  & \ding{51}   \\
 
  Anaphor \newline (Number) & 
    nan ~~dianyuan ~~~~~~~\textbf{men} kanjianle \textbf{tamen}-ziji.\newline male shop assistant \texttt{PL} ~~saw ~~~~~~~~~themselves\newline
    ``The male shop assistants ~saw themselves."& 
 nan ~~dianyuan ~~~~~~~men kanjianle ~~\textbf{ta}-ziji.\newline male shop assistant \texttt{PL} ~~saw ~~~~~~~~~himself &
 \ding{51} &           & \ding{51} &  & \ding{51}   \\
 \rowcolor{aliceblue}
 Aspect      & 
 ta ~\textbf{qu} ~nian zhiding ~~zhengce le.\newline he last year establish policy ~~~\texttt{AS}\newline
 ``He established policies last year."  & 
 ta ~\textbf{ming} nian zhiding ~~zhengce le.\newline he next ~~year establish policy ~~~\texttt{AS} & \ding{51}
  &   &            &     & \ding{51} \\

 Classifier-Noun & 
 yi ~~~\textbf{ming} tielu ~~~~~jingcha\newline one \texttt{M} ~~~~~~~railway policeman\newline 
 ``a railway policeman" & 
 yi ~~\textbf{tiao} tielu ~~~~jingcha\newline one \texttt{M} ~~~railway policeman &  & \ding{51} & \ding{51} & \ding{51} & \ding{51} \\
 \rowcolor{aliceblue}
 Definiteness Effect & 
 zheli/nali ~you ~~\textbf{yi} ~~jia yingyuan.\newline here/there exist one \texttt{M} ~cinema\newline
 ``Here/there exists a cinema." &  
 zheli/nali ~you ~~\textbf{zhe}/\textbf{na}/\textbf{mei} ~jia yingyuan.\newline here/there exist \texttt{DT}/\texttt{DT}/every \texttt{M} ~cinema & 
 &    \ding{51}    &     &    &  \\

 Polarity Item & 
 ta ~~\textbf{bu} ~fazhan ~~renhe youhao ~guanxi.\newline she not develop any ~~~friendly relations \newline
 ``She does not develop any friendly relations."  &
 ta ~~fazhan ~~renhe youhao ~guanxi.\newline she  develop any ~~~friendly relations &
            & \ding{51} &            &       &  \\
\rowcolor{aliceblue}
 Relative Clause  & 
 ta ~~jiandao le ~~na ge  zhizhi le ~baoli ~~~~~~de ~~~n{\"u} ~~~~~~jingcha.\newline
 she see ~~~~~~\texttt{AS} \texttt{DT} \texttt{M}  ~stop ~~\texttt{AS} violence \texttt{DEC} female police\newline
 ``She saw the female police officer who stopped the violence." &
 ta ~~jiandao le ~na ~ge \textbf{ta} ~zhizhi le ~baoli ~~~~~de ~~~~n{\"u} ~~~~~~~jingcha.\newline
 she see ~~~~~~\texttt{AS} \texttt{DT} \texttt{M} she stop ~~\texttt{AS} violence \texttt{DEC} female police & 
 \ding{51} &           &            &  & \ding{51} \\
 \textit{Wh}-fronting & 
 tamen shang ge yue ~~~~daodi ~~~~goujie ~~~~~~~~~~le ~~\textbf{shenme}?\newline they ~~~last ~~~~\texttt{M} ~month on earth collude with \texttt{AS} what\newline
 ``What on earth did they collude with last month?" & 
 \textbf{shenme} tamen shang ge yue ~~~~daodi ~~~~goujie ~~~~~~~~~~le?\newline  what ~~~~they ~~~last ~~~~\texttt{M} ~month on earth collude with \texttt{AS} &
 \ding{51} &           &            &     &   \\
\bottomrule
\end{tabular}}
\caption{Syn = syntax; Sem = semantics. An overview of the phenomena investigated in the current work. It indicates whether the paradigms under the phenomena represent syntax or semantics knowledge, whether they involve a distractor, whether there is long distance dependencies, and whether the LMs need hierarchy knowledge of the language to distinguish the acceptable and unacceptable sentences. }
\label{tab:overview_phenomena}
\end{table*}
















==> sections/relatedwork.tex <==
\section{Related Work}

% \subsection{Language models}

% \kkcomment{move this section to appendix}
% Language modeling uses statistical and probabilistic techniques to give a probability distribution of a vocabulary in a language. An early and simple probabilistic LM is \textit{n}-grams \citep{suen1979n}. \textit{N}-grams calculate the conditional probability of the \textit{n}-th word following a sequence of $n-1$ elements with \textit{n} being an integer bigger than zero. Later, \citet{elman1990finding} introduces recurrent neural networks 
% that makes language modeling effective. But RNN LMs are sequential which can be time-consuming and restricted to local dependencies. Recent year, the attention mechanism is proposed \citep{bahdanau2014neural,luong2015effective} and applied in language modeling by \citet{vaswani2017attention}. The resulting model, Transformer, breaks through the bottlenecks of RNN LMs: it is highly parallelizable and enhances global dependencies in sequences. Based on Transformer, two types of LMs are 
% constructed. The first type is causal LMs, represented by GPT-2 \citep{radford2019language} and GPT-3 \citep{brown2020language}. The training objective is to predict the next work given a prefix. The second LM type is masked LMs, for example, BERT \citep{devlin2018bert}. The training objective is to predict a masked token given the context surrounding that token. 

% Nowadays, LMs of different languages are available, as well as multi-lingual LMs. Each of them is useful in certain downstream tasks. However, it is not clear how much linguistic knowledge each LM has acquired. \yscomment{But why do we want to know that ...} Various methods have been proposed to evaluate LMs' linguistic knowledge. They will be reviewed below. 

\subsection{Methods of Evaluating Linguistic Knowledge}
% \kkcomment{While shortening, try to keep as many citations as possible, but you can make each citation less descriptive.. I've uncommented the first paragraph.. you could also add a sentence motivating why linguistic evaluation of LMs is important, and then say "This has led to development of several methods like ...". I think you can significantly shorten this section (preserving the citations), but keep the last paragraph or so motivating the need for minimal pair evaluations (they are general-purpose / applicable to any LM). You could also cite some probing BERTology papers here, like https://arxiv.org/abs/1905.05950, https://arxiv.org/abs/1905.06316, https://arxiv.org/abs/1906.04341}

To investigate what kind of and how much linguistic knowledge large-scale pre-trained LMs have compared to human, previous works have focused on limited LMs and probed into the internal encoding of the linguistic knowledge \citep{tenney2019bert, tenney2019you, clark2019does}. Other works investigate the LMs' linguistic knowledge of a small subset of English syntactic grammar by using prefix methods \citep{2016Linzen,2018Gulordava,2019Wilcox}, by-word surprisal \citep{2018Futrell}, or trained an acceptability classifier \citep{2019Warstadt}.

\citet{2016Linzen} focus on English subject-verb dependencies and use a prefix method for evaluation, which requires LMs assign probabilities to the next word given a prefix. The grammatical next word is expected to have a higher probability (e.g., \textit{The keys \textbf{are}} vs. *\textit{The keys \textbf{is}}). %The task includes local subject-verb dependencies (e.g., \textit{The keys \textbf{are}} vs. *\textit{The keys \textbf{is}}) as well as dependencies in distance with distractors (e.g., \textit{The roses in the \underline{vase} by the \underline{door} \textbf{are}} vs. *\textit{The roses in the \underline{vase} by the \underline{door} \textbf{is}}). The prefix method is adopted in later works, for example,  \citet{2018Gulordava} and \citet{2019Wilcox}.

Inspired by the controlled psycholinguistic experimentation, \citet{2018Futrell} applied by-word surprisal\footnote{Surprisal is the log inverse probability of a word given its prefix \citep{hale2001}.} and sentence completion methods to explore LMs' knowledge of syntax. %The by-word surprisal method is used to probe LMs' expectation of certain words given a context. 
The surprisal reflects whether LMs are affected by the presence/absence of critical words in grammatical configurations. In the sentence completion task, LMs completes a sentence given a prefix. Human annotators then judge the grammaticality of the completed sentences. 

\citet{2019Warstadt} trained an acceptability classifier to perform a grammaticality judgement task, which consists of sentences collected from the linguistics literature marked for their acceptability. 

These methods are either only applicable to a subset of linguistic grammar (mainly syntax) or depend on the performance of a classifier. The minimal pair method used in BLiMP breaks through these limitations. 

\subsection{BLiMP}

To cover a wide range of linguistic phenomenon, \citet{blimp} introduced minimal pair evaluation for LMs, which is a common practice in linguistics study for acceptability judgement. An acceptable sentence should be assigned a higher probability than its unacceptable counterpart. 

BLiMP evaluates the linguistic knowledge of twelve English grammatical phenomena including syntax and semantics. Each of them consists of minimal pair paradigms representing different aspects of the phenomena. All minimal pairs are code-generated using templates created by linguists and an annotated vocabulary that contains 3000 words. The dataset is human validated. %A subset of the minimal pairs is validated by English native speakers. The validation task is to choose the better sentence in a minimal pair. Twenty annotators evaluated 5 minimal pairs from each paradigm. Using the majority vote, human accuracy is 96.4\%. 

It is shown that the LMs tested in BLiMP are good at local dependency relations (e.g., morphology agreement) but bad at phenomena involving hierarchy and semantic knowledge. %The accuracy on short sentences tends to be higher than the one on long sentences. 
Concerning the training size and model size, while increasing training size can improve model performance, increasing model size does less so. %\kkcomment{Can cut some sentences like human validated, results on training/model size.. You could move these sentences to your results section --- something like "In SLING we observe model size does not necessarily lead to improvements. A similar finding was seen in BLiMP".. and in the section you describe your human annotation, you can say how it's similar / different from BLiMP's evaluation. In this section try to only introduce the dataset and the task setup.}

% There are four language models tested in BLiMP. Two of them use the Transformer architecture: 
% \vspace{-0.1\baselineskip}
% \begin{itemize}
%     \item GPT-2 \citep{radford2019language}
%     \vspace{-0.5\baselineskip}
%     \item Transformer-XL \citep{dai2019transformer}
% \end{itemize}
% \vspace{-0.1\baselineskip}
% \noindent and the other two are:
% \vspace{-0.1\baselineskip}
% \begin{itemize}
%     \item LSTM \citep{gulordava2018colorless}
%     \vspace{-0.5\baselineskip}
%     \item 5-gram LM trained on the English Gigaword corpus \citep{graff2003english}
% \end{itemize}
% \vspace{-0.1\baselineskip}
% To estimate the relation of training size and model performance, \citet{blimp} train a series of LSTM and Transformer-XL models using the same hyperparameters but different training sizes. 

% The accuracy of the language models is the proportion of the minimal pairs in which the models give the acceptable sentences a higher probability. Among the four types of language models, GPT-2 performs the best and the 5-gram the worst. Overall,  \kkcomment{Can cut down the summary of BLIMP results since it's not directly relevant to SLING}

% \subsection{CLiMP}

% Following the procedure of BLiMP, \citet{climp} created CLiMP, which covers nine Chinese phenomena with 16 paradigms. The vocabulary is translated from BLiMP along with the  morphological, syntactical, and semantic annotations. 456 annotated words that are specific to Chinese are added, resulting in a 3456 word vocabulary. The majority vote human agreement with the sentence labels is 97.1\%. CLiMP tests bert-base-chinese, three LSTM LMs, and two 5-gram LMs. The performance of the language models is based on the proportion of the minimal pairs in which the models give the acceptable sentences a lower perplexity \citep{gulordava2018colorless}. For the masked LM, pseudo-perplexity is used instead \citep{salazar2019masked}. The results of CLiMP shows that bert-base-chinese largely outperforms the other LMs. The LMs are good at classifier–noun agreement and verb complement selection but bad at \textit{ba} construction, binding, and filler-gap dependencies. The authors conclude that the LMs are bad at long-distance dependencies, and the lack of hierarchical knowledge is the reason for it. Even though most of their LMs perform close to chance, the authors find that larger training size occasionally lead to better performance in the LSTM and 5-gram models. 

% % \vspace{-0.1\baselineskip}
% % \begin{itemize}
% %     \item bert-base-chinese \citep{devlin2018bert}
% %     \vspace{-0.5\baselineskip}
% %     \item LSTM LMs trained on 0.4M, 2M, and 21.5M sentences from Chinese Wikipedia with word-based and character-based tokenizers \citep{dai2019transformer}
% %     \vspace{-0.5\baselineskip}
% %     \item 5-gram LMs trained on 0.4M and 2M sentences from Chinese Wikipedia with word-based and character-based tokenizers
% % \end{itemize}
% % \vspace{-0.1\baselineskip}

% As the first benchmark for the evaluation of linguistic knowledge in Chinese LMs, CLiMP covers grammar phenomena that do not occur in English. However, it does not provide a view of how modern large-scale LMs perform with respect to Chinese linguistic phenomena. Moreover, CLiMP has two major problems with their minimal pair generation. 

% \paragraph{CLiMP vocabulary has low diversity.} The foremost problem is that their vocabulary is translated from BLiMP but a lot of annotated features of BLiMP do not apply to Chinese (e.g., number features, verb forms, or cases). This causes CLiMP's vocabulary being repetitive. As an example, the verb \textit{buy} has six entries, listed in Table \ref{tab:climprepetitive}. The entries differ from each other in seven verb-related features. However, the same entries can be represented and built based on the three words in bold: \textit{mai} (buy), \textit{(zheng)zai} (progressive marker), and \textit{le} (perfective marker). With the presence of the latter two, every verb only needs one entry. The others can be built accordingly. The same repetition problem applies to nouns for the number feature as well. After removing the repetitive entries, the vocabulary size is 1272 (including 230 proper names), which is much smaller than it is claimed to be. 

% \begin{table}[!h]
% \centering
% \begin{tabular}{@{}lll@{}}
% \toprule
% Chinese & English & Features\\
% \midrule
% \textbf{mai}           & buy  & bare \\
% \textbf{zheng zai} mai & buying & ing\\
% mai \textbf{le}        & bought & finite, past\\
% mai le        & bought & en \\
% mai           & buy    & finite, pres\\
% mai           & buys   & finite, pres, 3sg \\ 
% \bottomrule
% \end{tabular}
% \caption{An example of the repetitive entries in CLiMP's vocabulary. The third column contains the features that distinguish the expressions. Feature meaning: ing = progressive, en = participle, pres = present, 3sg = third person singular.}
% \label{tab:climprepetitive}
% \end{table}

% \paragraph{CLiMP has inadequately designed minimal pairs.} First, the contrast in the minimal pairs is not always clear. It is because of the inadequacy of the vocabulary as well as the templates, especially the ones of the \textit{ba} construction, binding/anaphor, and filler-gap dependency, which are the ones that the LMs are claimed to be bad at. Concerning the \textit{ba} construction, the template contrasts \textit{ba} to \textit{bei} (i.e., active \textit{vs.} passive voice), attempting to test whether the LMs understand theta roles. However, the theta role related information is not sufficiently annotated in the vocabulary, resulting in the lack of clear contrast in the minimal pairs. %Nonetheless, admittedly, the characteristics of the \textit{ba} construction are hard to capture and go beyond verb selection. It is still a pending question for theoretical linguistics \citep{li2017chinese}. 
% The issues in the binding and anaphor paradigms is that CLiMP uses proper names which do not unambiguously show the gender. It also do not exclude the influence of gender bias in LMs. The issues of the minimal pair design are presented in Section \ref{subsec.anaphor}. For the filler-gap paradigm, the authors claim that they use what they call topicalization construction. Example (\ref{ex.fillergap}a) is taken from CLiMP which is supposed to be good. However, it is not a filler-gap topicalization dependency at all. A real topicalization filler-gap structure should be the one in (\ref{ex.fillergap.real}b), in which the direct object of the verb \textit{buy} is moved to the front of the sentence, leaving an empty category \textit{t}\textsubscript{1} at its base generated position. 

% \begin{exe}
% \small
%     \ex\label{ex.fillergap}
%     \begin{xlist}
%     \ex
%     \gll men, wo mai le zhe dongxi.\\
%         door, I buy \texttt{AS} \texttt{DT} thing\\
%     \glt ``Door, I bought this thing."
    
%     \ex\label{ex.fillergap.real}
%     \gll men\textsubscript{1}, wo mai le \textit{t}\textsubscript{1}.\\
%         door, I buy \texttt{AS}\\
%     \glt ``Door, I bought."
%     \end{xlist}
% \end{exe}

% % Besides the two major issues in the minimal pair design, . It tests multiple versions of LSTM and 5-gram LMs but only one masked LM. To gain a better understanding of the performance of modern LMs, the current work includes the majority of the available Chinese causal and masked LMs.



